Generalized Direct Change Estimation in Ising Model Structure

We consider the problem of estimating change in the dependency structure between two $p$-dimensional Ising models, based on respectively $n_1$ and $n_2$ samples drawn from the models. The change is assumed to be structured, e.g., sparse, block sparse, node-perturbed sparse, etc., such that it can be characterized by a suitable (atomic) norm. We present and analyze a norm-regularized estimator for directly estimating the change in structure, without having to estimate the structures of the individual Ising models. The estimator can work with any norm, and can be generalized to other graphical models under mild assumptions. We show that only one set of samples, say $n_2$, needs to satisfy the sample complexity requirement for the estimator to work, and the estimation error decreases as $\frac{c}{\sqrt{\min(n_1,n_2)}}$, where $c$ depends on the Gaussian width of the unit norm ball. For example, for $\ell_1$ norm applied to $s$-sparse change, the change can be accurately estimated with $\min(n_1,n_2)=O(s \log p)$ which is sharper than an existing result $n_1= O(s^2 \log p)$ and $n_2 = O(n_1^2)$. Experimental results illustrating the effectiveness of the proposed estimator are presented.

==> related.tex <==
\ff{{\color{red} not ready: both writing and content - will finish it at the end}}

\ab{do we need a separate section? can we move important stuff to the discussion in the intro?} 

Multi-task learning is developed to jointly estimate paramters $\theta_1$ and $\theta_2$ by assuming that they share a common sub-structure~\cite{daww14,glmz11,hawa11,hosa10,mlfw14}.
% Several multi-task graphical models have been proposed to estimate multiple graphical models simultaneously which capture the similarity between graphical models using a Fused type lasso penalty~\cite{daww14,glmz11,hawa11,hosa10} or perturbed node penalty~\cite{mlfw14}.
While multi-task graphical models allow for an efficient use of training data, these models lack the theoretical guarantees on the estimated changes and assume that both $\theta_1$ and $\theta_2$ are sparse. In particular, these models are inefficient in high-dimensional setting especially if the difference between two graphs is sparse while the individual graphs are dense. %since the sample complexity of graphical models depends on the sparsity level~\cite{baga08,kahs09,mebu06,rawl10,rwry11,yglr12}.

%Why Density Ratio for Change Detection
Recently, Liu et~al.~\yrcite{lqgs14} proposed a direct estimator for the changed estimation problem based on the density ratio techniques \cite{gshs09,kahs09,snkp08,vaiz15} without estimating the individual dependency graphical model structures.
%~Consider two set of samples $\{X_i^p\}_{i=1}^{n_p}$ and $\{X_i^q\}_{i=1}^{n_q}$ generated from two exponential family distributions $p(X|\theta_p^*)$ and $q(X|\theta_q^*)$, respectively. Then, the density ratio $p(X|\theta_p^*)/q(X|\theta_q^*)$ directly encodes the changed edges  between two networks~($\theta^* = \theta_p^*-\theta_q^*$).
Liu et~al.~\yrcite{lqgs14} formulated a regularized optimization where the loss function is defined based on the density ratio and the optimal parameter $\delta \theta^*$ is assumed to be sparse. Later, Liu et~al.~\yrcite{liss14} showed the non-asymptotic error bound for such estimator~\cite{lqgs14} which requires the sample complexity of $n_1=O(s^2 \log p)$ and $n_2=O(s^3 \log^2 p)$ where $s$ is the number of the changed edges, and $p$ is the parameter dimensionality.

In another work, Zhao et~al.~\yrcite{zhcl14} estimated the direct changes in Gaussian graphical models by solving a constrained optimization problem and defining the differential graphical model structure as the difference between the two precision matrices (inverse of covariance matrix) at each state. Under the assumption that $\delta
\theta^*$ is sparse, Zhao et~al.~\yrcite{zhcl14} show that the direct estimator is consistent in support
recovery and estimation but their model is only applicable to Gaussian graphical models not Ising models.
However, both models~\cite{liss14,zhcl14} assumed that $\delta \theta^*$ can only be sparse and their analysis can not be applied for problems where $\delta \theta^*$ has a different structure such as group-sparse.




==> theo-lambda.tex <==
As discussed in Section \ref{sec:anal-back}, the regularization parameter $\lambda$
needs to satisfy the following inequality,
\begin{align}
\lambda > \beta R^*(\nabla \cL(\theta^{*})),
\label{eq:lam}
\end{align}
for $\beta > 1$. 
Note that the expression \eqref{eq:lam} is a random expression which also depends on an unknown parameter $\theta^*$. In this section, we provide an upper bound on $R^*(\nabla \cL(\theta^{*}))$ in terms of the Gaussian width of the unit norm ball and also charecterize its expectation.

Note that the loss function \eqref{eq:losschangedet} depends on two sets of samples. From the definition, we have
\begin{align}
\nabla \cL(\theta^*) &= \frac{-1}{n_p} \sum_{i=1}^{n_p} T(X_i^p)  + \nabla \hat{\Psi}(\theta^*),
\end{align}
where $\nabla \hat{\Psi}(\theta^*)$ only depends on samples from $q$.
Therefore, to obtain the bound on $R^*(\nabla \cL(\theta^{*}))$, we apply triangle inequality property of norms as
\begin{align}
R^*(\nabla \cL(\theta^*)) \leq R^*(\frac{-1}{n_p} \sum_{i=1}^{n_p} T(X_i^p)  )+ R^*(\nabla \hat{\Psi}(\theta^*)).
\end{align}
Now we break down the analysis on two steps by bounding $R^*(\frac{-1}{n_p} \sum_{i=1}^{n_p} T(X_i^p) )$ and $R^*(\nabla \hat{\Psi}(\theta^*))$ separately as follows.

 \begin{theo}
Consider sufficient statistic $T(X_i^p)$ for all $i = 1, \cdots n_p$ where $n_p$ samples $\{X_i^p\}_{i=1}^{n_p}$ are independent. Define $\Omega_R = \{u: R(u) \leq 1\}$. 
Then, 
\begin{align}
E\left[R^*(\frac{1}{n_p} \sum_{i=1}^{n_p} T(X_i^p)))\right] \leq \frac{c_1}{\sqrt{n_p}} w(\Omega_R).
\end{align}
and with probability at least $1-\eta_0 e^{-\epsilon^2}$
\begin{align}
R^*\left(\frac{1}{n_p} \sum_{i=1}^{n_p} T(X_i^p) \right) \leq \frac{\eta_3}{\sqrt{n_p}} w(\Omega_R),
\end{align}
where $w(\Omega_R)$ is the Gaussian width of set $\Omega_R$, $\eta_3$, $\eta_2$, and $\eta_0$ are positive constant depends on $\epsilon$.
 \label{theo:BndLambdaXp}
 \end{theo}
 
 \begin{theo}
Consider sub-Gaussian sufficient statistic $T(X_i^q)$ where samples $\{X_i^q\}_{i=1}^{n_q}$ are independent.
Let $\hat{\Psi}(\theta^*) = \log \frac{1}{n_q} \sum_{i=1}^{n_q} \exp\{ \langle T(X_i^q), \theta^* \rangle \}$.
Define $\Omega_R = \{u: R(u) \leq 1\}$.
% Let
% \beq
% = R^*\left( \sum_{i=1}^{n_q} T(X_{i}^q) \hat{r}(X_i|\theta) - E_{X\sim q}[T(X)r(X|\theta^*)]\right)
% \eeq
Then, we have
\begin{align}
E\left[R^*\left(\nabla \hat{\Psi}(\theta^*) \right)\right] \leq c_0 w(\Omega_R),
\end{align}
and with probability at least $1-\eta_0 \exp\{-\epsilon^2\}$, we have
\begin{align}
R^*\left(\nabla \hat{\Psi}(\theta^*)\right) \leq \frac{\eta_3}{\sqrt{n_q}^{1-\alpha}} w(\Omega_R),
\end{align}
where $w(\Omega_R)$ is the Gaussian width of the set $\Omega_R$, and $c$, $c_0$, $c_1$, $\eta_0$, $\eta_1$, and $\eta_3$ are positive constant depending on $\epsilon$.
 \label{theo:BndLambdaXq}
 \end{theo}

Putting the results of Theorem \ref{theo:BndLambdaXp} and \ref{theo:BndLambdaXq} together, we know able to provide the bound on $R^*(\nabla \cL(\theta^*))$.
\begin{theo}
Consider sufficient statistic $T(X_i^q)$ and $T(X_i^p)$ with independent samples $\{X_i^p\}_{i=1}^{n_p}$, $\{X_j^p\}_{j=1}^{n_p}$.
Define $\Omega_R = \{u: R(u) \leq 1\}$. Then, with probability at least $1- e \cdot \exp\left( -\eta_1 \log n \right)$
\begin{align}
\hspace{-0.4cm} E[R^*(\nabla \cL(\theta^{*}))] \leq \frac{c_1}{\sqrt{n_p}} w(\Omega_R) + \frac{c_2}{\sqrt{n_q}} w(\Omega_R),
\label{eq:expsubgwidthpq}
\end{align}
and with probability at least $1-\eta_0 e^{-\epsilon} - e \cdot \exp\left( -\eta_1 \log n \right)$,
 \begin{align}
  R^*(\nabla \cL(\theta^{*})) & \leq  \frac{\eta_2}{\sqrt{n_p}} w(\Omega_R) + \frac{\eta_2}{\sqrt{n_q}} w(\Omega_R),
 \end{align}
 where $w(\Omega_R)$ is the Gaussian width of set $\Omega_R$, for small value $\alpha = \frac{2c}{\sqrt{\log n}}$, and $c_1$, $c_2$, $\eta_3$, $\eta_2$, and $\eta_0$ are positive constant depends on $\epsilon$ and $K$.
 \label{theo:lambdabnd}
\end{theo}

The proof is given in the supplement.

{\bf Remark 1: } In the proof of Theorem \ref{theo:lambdabnd}, we assume that the sufficient statistic $T(X)$ is suitably truncated; similar assumption is made in consistency analysis of graphical models~\cite{yang2013poisson,yglr12}. Note that, for bounded random variables $T(X)$ is bounded which satisfies our assumption. An example of bounded random variables is Ising model which $X^i \in \{-1, 1\}$ for all random variables, and $T(X)_{i,j} = X^i X^j$. This model is used in many applications of spatial statistics such as modeling the behavior of gases or magnets in statistical physics, building statistical models in computer vision and social network analysis.
A similar assumption is also considered in previous analysis of density ratio estimator~\cite{liss14} by assuming that $\exp \{\langle T(X), \theta \rangle - \Psi(\theta)\}$ has sub-Gaussian tail which is only possible when $T(X)$ is bounded or suitably truncated.


{\bf Remark 2: } If $R(.)$ is the $\ell_1$ norm, then with high probability we have the bound
\beq
R^*(\nabla \cL(\theta^{*})) \leq \left( \frac{\eta_2}{\sqrt{n_p}} + \frac{\eta_2}{\sqrt{n_q}} \right) \sqrt{\log p}.
\label{eq:lambdaL1}
\eeq

{\bf Remark 3: } If $R(.)$ is the group-sparse norm, then with high probability we  have the bound
\beq
R^*(\nabla \cL(\theta^{*})) \leq \left( \frac{\eta_2}{\sqrt{n_p}} + \frac{\eta_2}{\sqrt{n_q}} \right) \sqrt{m+\log N_G}.
\label{eq:lambdaGroup}
\eeq


% \proof
% Let $Z \in \R^{n_q \times d}$ with each row $Z_i = T(X_{i}^q)$ is a sub-Gaussian vector with $\vertiii{Z_i}_{\Psi_2} < K$. Define $\sigma =\{\sigma_i\}_{i=1}^{n_q} \in \R^{n_q}$ with each element $\sigma_i = \frac{\exp\{ \langle Z_i, \theta \rangle \}}{\sum_{j=1}^{n_q}  \exp\{ \langle Z_j, \theta \rangle \}} $.
% Using the definition of the dual norm, we have 
% \begin{align}
% R^*\left(\frac{1}{n_q}\sum_{i=1}^{n_q}  T(X_{i}^q) ~\hat{r}(X_i^q|\theta) - E_{X\sim q}[T(X)r(X|\theta^*)] \right) = R^*\left(Z^T \sigma - E[Z^T \sigma]\right) \\
% = \|\sigma\|_2  \sup_{u \in \Omega_R} \left \langle {Z}^T \frac{\sigma}{\|\sigma\|_2}-E[Z^T \frac{\sigma}{\|\sigma\|_2}], u  \right \rangle.
% \label{eq:dualRqbnd}
% \end{align}
% 
% We bound \eqref{eq:dualRqbnd} in two steps: 
% \begin{enumerate}
%  \item Get an upper bound for $\|\sigma\|_2$ by applying Lemma \ref{lem:bndSig}. In particular, using the definition of $\sigma_i$ and applying a union bound, we show that with probability at least $1 -e \cdot \exp\left( - \eta_1 \tau^2 -\log n) \right)$,
%  \begin{align}
% \frac{e^{-2\tau}}{\sqrt{n_q}} \leq \|\sigma\|_2 \leq \frac{e^{2\tau}}{\sqrt{n_q}},
% \end{align} 
% where $\eta_2=\frac{1}{4\|\theta\|_2K}$ is a positive constant.
% \item Get an upper bound on $\sup_{u \in \Omega_R} H(u)$ where $H(u) = \left \langle {Z}^T \frac{\sigma}{\|\sigma\|_2}-E[Z^T \frac{\sigma}{\|\sigma\|_2}], u  \right \rangle$ by applying Lemma \ref{lem:subGaussianWidthGaussianWidthq}. In particular, we show that the process $H(u)$ is a centered sub-Gaussian process and applying an application of generic chaining with theorem \ref{theo:FertalsubGau} \cite[Theorem  8.2 (Fernique-Talagrand's  comparison  theorem)]{vers14}, with probability at least $1-\eta_0 \exp\{- \epsilon\} - e \cdot \exp\left( -\eta_1 \tau^2 -\log n\right)$, we have
% \begin{align}
% \sup_{u \in \Omega_R} H(u) \leq \eta_2 w^2(\Omega_R)+ \eta_3 w(\Omega_R),
% \end{align}
% where $w(\Omega_R)$ is the Gaussian width of the set $\Omega_R$, and $\eta_0$, $\eta_1$, and $\eta_3$ are positive constat depending on $\epsilon$ and $K$.
% \end{enumerate}
% 
% Set $\tau = c \sqrt{\log n}$. This completes the proof.
% \qed



% % 
% % \begin{align*}
% % P \left[\left| \langle \frac{\sigma}{\|\sigma\|_2}, Zu \rangle \right| \geq \tau \right] 
% % &= P \left[\left|\sum_{i=1}^{n_q} \frac{\sigma_i}{\|\sigma\|_2} \langle Z_i, u \rangle \right| \geq \tau \right] \\
% % & \leq \sum_{i=1}^{n_q} P\left[ \left| \frac{\sigma_i}{\|\sigma\|_2}\right| \geq \frac{\sqrt{\tau}}{\sqrt{n_q}}  \right] 
% % + P \left[\left|\langle Z_i, u \rangle \right| \geq \frac{\sqrt{\tau}}{\sqrt{n_q}}  \right] \\
% % & \leq \sum_{i=1}^{n_q} e. \exp\{-\frac{\tau}{c^2}\} + e. \exp\{ -\frac{\tau}{K^2 n_q \|u\|_2^2} \} \\
% % &\leq e. \exp\{- (\eta_0 \tau - \log n_q) \} + e. \exp\{ - (\eta_1 \tau - \log n_q)\} \\
% % & \leq 2 e. \exp\{- [ \min (\eta_0, \eta_1) \tau - \log n_q ] \} \\
% % & = 2 e. \exp\{- (\frac{\tau}{K_1} - 1) \},
% % \end{align*}
% % where $\eta_0 = \frac{1}{c^2}$ and $\eta_1 = \frac{1}{K^2 n_q \|u\|_2^2}$, 
% % \begin{align}
% %  K_1 = \frac{\log n_q}{\min (\eta_0, \eta_1)} = \frac{\log n_q}{\min(\frac{1}{c^2},\frac{1}{K^2 n_q \|u\|_2^2})} = \max (c^2, K^2 n_q \|u\|_2^2) \log n_q
% % \end{align}
% 
% %Note that $E[w_i] = \frac{\sum_{i=1}^{n_q} w_i}{n_q} = \frac{1}{n_q}$. Given that $w_i$ is bounded, $h_i = w_i - E[w_i]$ is a centered sub-Gaussian variable with $\vertiii{h_i}_{\Psi_2} < \frac{1}{2n_q\beta^2}$. As a result, $h_i^2$ is a  sub-exponential variable with $\vertiii{h_i^2}_{\Psi_1} < \frac{1}{4n_q^2\beta^4}$.
% %Since $w_i$ are dependent, elements of $h$ are dependent. As a result, we have $\vertiii{\sum_{i=1}^{n_q} h_i^2}_{\Psi_1} < n_q\frac{1}{4n_q^2\beta^4} = \frac{1}{4n_q\beta^4} $ {\color{red} check if it is true! In particular if $X_1$ and $X_2$ are dependent sub-exponential random variable with $\vertiii{X_1}_{\Psi_1}=\vertiii{X_2}_{\Psi_1} = K$, then $X_1+X_2$ is a sub-exponential random variable with $\vertiii{X_1+X_2}_{\Psi_1} = 2K$.}.
% %
% %Applying the concentration bound on sub-exponential random variable, we have
% %\beq
% %p \left (|\sum_{i=1}^{n_q} h_i^2 - E[\sum_{i=1}^{n_q} h_i^2]| > \epsilon ~~\Big |~~ |\langle Z_i, \theta_r \rangle| < \tau \right) \leq \exp \left\{ 1- 4\epsilon n_q \beta^4 \right \}
% %\eeq
% %Setting $\epsilon = \frac{1}{\beta^4 n_q}$, we have
% %
% %\beq
% %p \left (|\sum_{i=1}^{n_q} h_i^2 - E[\sum_{i=1}^{n_q} h_i^2]| > \frac{1}{\beta^4 n_q} ~~\Big |~~ |\langle Z_i, \theta_r \rangle| < \tau \right) \leq \exp \left\{ -3 \right \}
% %\eeq
% %
% %As a result,
% %\beq
% %p \left (|\sum_{i=1}^{n_q} h_i^2-E[\sum_{i=1}^{n_q} h_i^2]| > \frac{1}{\beta^4 n_q} \right) \leq e^{-2} \cdot \exp\left( - \frac{c_1 \tau^2}{K^2 \| \theta_r \|^2} \right)
% %\eeq
% %
% %Bound on $E[\sum_{i=1}^{n_q} h_i^2]$:
% %\beq
% %E[\sum_{i=1}^{n_q} h_i^2] = \frac{-1}{n_q} + \sum_{i=1}^{n_q} E[w_i^2] \leq \frac{-1}{n_q} + \frac{1}{2n_q\beta^4}
% %\eeq
% %where the last inequality obtain by using the fact that $w_i$ is a sub-Gaussian with $\vertiii{w_i}_{\Psi_2} < \frac{1}{2n_q\beta^2}$, therefore $E[w_i^2] < 2 \frac{1}{4n_q^2\beta^4} = \frac{1}{2n_q^2\beta^4}$.
% %
% %
% %Since $\sum_{i=1}^{n_q} h_i^2 = \sum_{i=1}^{n_q} (w_i-E[w_i])^2 =  \sum_{i=1}^{n_q} [w_i^2 + \frac{1}{n_q^2} - 2\frac{w_i}{n_q}] =  \sum_{i=1}^{n_q} [w_i^2] - \frac{1}{n_q} $, we have
% %\beq
% %p \left (\frac{1}{n_q} - \frac{1}{\beta^4 n_q} \leq \sum_{i=1}^{n_q} w_i^2 \leq \frac{1}{n_q}+\frac{1}{\beta^4 n_q} \right) \geq 1- e^{-2} \cdot \exp\left( - \frac{c_1 \tau^2}{K^2 \| \theta_r \|^2} \right)
% %\eeq
% 
% %\beq
% %p \left (|\sum_{i=1}^{n_q} h_i^2| > \frac{1}{\beta^4 n_q} \big| |\langle Z_i, \theta_r \rangle| < \tau  \right) \leq 2 \exp \left\{ -\min \left( \frac{16 n_q^4 \beta^8}{\beta^8 n_q^3}, \frac{4n_q^2 \beta^4}{\beta^4 n_q}  \right) \right \} = 2 \exp \left\{-4 n_q \right \}
% %\eeq
% 
% %As a result, we have with probability at least  $1-e \cdot \exp\left( - \frac{c \tau^2}{K^2 \| \theta_r \|^2} \right)$
% %\begin{align}
% %p \left( \frac{\beta^2}{n_q} \leq w_i \leq \frac{1}{n_q\beta^2} \right) > 1-e \cdot \exp\left( - \frac{c \tau^2}{K^2 \| \theta_r \|^2} \right) \\
% %p \left( \frac{\beta^4}{n_q^2} \leq w_i^2 \leq \frac{1}{n_q^2\beta^4} \right) > 1-e \cdot \exp\left( - \frac{c \tau^2}{K^2 \| \theta_r \|^2} \right) 
% %\end{align}
% %
% 
% 
% % Therefore,
% % \begin{align}
% % E\left[R^*\left(\nabla \cL(\theta^{*}) \right)\right] \leq \Psi(\Omega_R) \{ \frac{1}{n_p} \sum_{i=1}^{n_p} c_1 w(\Omega_R) + \sum_{i=1}^{n_q} c_1 w(\Omega_R)\} = (1+n_q) \Psi(\Omega_R) w(\Omega_R).
% % \end{align}
% % That completes the proof.
% % \qed
% 
% % \begin{lemma}
% % Let $h \in \R^{p}$ be a sub-Gaussian vector with $\vertiii{h}_{\Psi_2} \leq K$ and $\Psi(A) = \sup_{u \in A} \frac{\|u\|_1}{\|u\|_2}$. Then
% % \begin{align}
% % E\left[ \sup_{u \in A} \left \langle h, u \right\rangle \right] \leq c_1 \Psi(A) E\left[ \sup_{u \in A} \left \langle g, u \right\rangle \right] = c_1 \Psi(A) w(A),
% % \end{align}
% % where $g \sim N (0, I_{{p^2} \times {p^2}})$ is standard Gaussian vector, and $w(A)$ is the Gaussian width of set $A$, and $c_1$ is a constant depending on $K$.
% % \label{lem:subgausswidth}
% % \end{lemma}
% % 
% % \proof
% % Consider the sub-Gaussian process $H(u) = \langle u, h \rangle$ indexed by $u \in A$. 
% % Consider the Gaussian process $G(u) = \langle u, g \rangle$, indexed by the same set, i.e., $u \in A$. First, note that $h_s = \langle h, s \rangle$ is a sub-Gaussian variable with $\vertiii{h_s}_{\psi_2} \leq K \|s\|_1$. So that by sub-Gaussian norm property, we have
% % \begin{align}
% %  \vertiii{H(u)-H(v)}_{\psi_2} &= \| u-v \|_1 \vertiii{\langle h, \frac{u-v}{\| u-v \|_1} \rangle}_{\psi_2} \nonumber \\
% %  & \leq K \| u - v \|_1 = K  \frac{\| u - v \|_1}{\| u - v \|_2} E_g[ \| G(u) - G(v) \|_2^2]^{1/2}.
% % \end{align}
% % where $E_g[ \| G(u) - G(v) \|_2^2]^{1/2} = E_g[\| \langle u-v , g \rangle\|_2^2]^{1/2} = \| u - v \|_2$.
% % 
% % Applying the Fernique-Talagrand's comparison theorem in Vershynin 2014 [], we have
% % 
% % \begin{align}
% % E\left[ \sup_{u \in A} \left \langle h, u \right\rangle \right] = E[\sup_{u\in A} H(u)] \leq c_2 K \Psi(A) E[ \sup_{u\in A} G(u)] =  c_1 \Psi(A) w(A),
% % \end{align}
% % where $c_1 = c_2 K$ with a positive constant $c_2$. That completes the proof.
% % \qed
% % 
% % \textbf{Remark 1:}
% % For set $A = \{u: \|u\|_1 \leq 1\}$, we have $\Psi(A)=1$ and $M = K$. Therefore, 
% % \[E\left[ \sup_{u \in A} \left \langle h, u \right\rangle \right] \leq K w(A) = O(\sqrt{\log p}).\]
% % 
% % \textbf{Remark 2:}
% % For set $A = \{u: \|u\|_2 \leq 1\}$, we have $\Psi(A)= \sqrt{p}$ and $M = K\sqrt{p}$. Therefore, 
% % \[E\left[ \sup_{u \in A} \left \langle h, u \right\rangle \right] \leq K \sqrt{p} w(A) = O(p).\]
% 
% 
% 
% % \begin{lemma}
% % Let $Z = \{Z_i\}_{i=1}^n \in \R^{n \times p}$ with independent rows and $Z_i$ are  sub-Gaussian vector with $\vertiii{Z_i}_{\Psi_2} \leq K$ and $\Psi(A) = \sup_{u \in A} \frac{\|u\|_1}{\|u\|_2}$. Let $Z_u^i = \sup_{u \in A} \langle Z_i, u \rangle $ is a sub-Gaussian process with $\vertiii{Z_u^i }_{\Psi_2} \leq K \Psi(A)$. Then, we have
% % \begin{align}
% % P\left(\frac{1}{n} \sum_{i=1}^n \left( Z_u^i - E\left[ Z_u^i \right] \right) > \tau \right) \leq e. \exp\{ - \frac{\tau^2 n^2}{K^2 \Psi^2(A)}\}.
% % \label{eq:hoffedingDeptsubGaussian}
% % \end{align}
% % \label{lem:subgausswidth}
% % \end{lemma}
% % 
% % \proof
% % Note that since components of $Z_i$ are dependent, then $\langle Z_i, u \rangle$ is a sub-Gaussian variable with norm
% % \beq
% % \vertiii{\langle Z_i, u \rangle}_{\Psi_2} \leq K \|u\|_1.
% % \eeq
% % As a result, 
% % \beq
% % \sup_{u \in A} \vertiii{\langle Z_i, u \rangle}_{\Psi_2} \leq \sup_{u \in A} K \|u\|_1 = K \Psi(A).
% % \eeq
% % Then \eqref{eq:hoffedingDeptsubGaussian} is obtained by applying concentration bound on independent sub-Gaussian variables.
% % 
% % \textbf{Remark 3:}
% % For set $A = \{u: \|u\|_1 \leq 1\}$, we have $\Psi(A)=1$. Therefore,  
% % \begin{align}
% %  p\left( \frac{1}{n} \sum_{i=1}^n  \left \{ \sup_{u \in A} \left \langle Z_i, u \right\rangle - E\left[ \sup_{u \in A} \left \langle Z, u \right\rangle \right] \right \} > \sqrt{\frac{\log p}{n}} \right) \leq e. \exp\{ - \frac{n \log p}{K^2}\}.
% % \end{align}
% % 
% % Hence,
% % \begin{align}
% %  p\left( \frac{1}{n} \sum_{i=1}^n \sup_{u \in A} \left \langle Z_i, u \right\rangle > \sqrt{\frac{\log p}{n}} + E\left[ \sup_{u \in A} \left \langle Z, u \right\rangle \right] \right) \leq e. \exp\{ - \frac{n \log p}{K^2}\} \\
% %   p\left( \frac{1}{n} \sum_{i=1}^n \sup_{u \in A} \left \langle Z_i, u \right\rangle > \sqrt{\frac{\log p}{n}} + \sqrt{\log p} \right) \leq e. \exp\{ - \frac{n \log p}{K^2}\} 
% % \end{align}
% 
% 
% 
% 
% %\newpage
% %%Note that, $\bar{Y}_i \in \{0, [e^{-T}, e^T]\}$. Define $\beta = e^{-T}$. Therefore, $\bar{Y}_i}$ is a bounded sub-Gaussian random variable with $\vertiii{\bar{Y}_i}_{\Psi_2} \leq \frac{1}{\beta}$.
% %%Define $\delta_j =\bar{Y}_i - E[\bar{Y}_i]$, where $\vertiii{\delta_i}_{\Psi_2} \leq \frac{2}{\beta}$.
% %% Similarly.
% %% \begin{align}
% %%  P(\exp\{\langle Z_i, \theta \rangle \} \I(|\langle Z_i, \theta \rangle| \leq T) = e^y) &= \frac{P\left(\exp\{\langle Z_i, \theta \rangle\} = e^y\right) \I(|\langle Z_i, \theta \rangle| \leq T)}{P\left(|\langle Z_i, \theta \rangle| \leq T\right)} \\
% %%  & \leq \frac{1}{1-\phi} P\left(\exp\{\langle Z_i, \theta \rangle \} = e^y\right).
% %% \end{align}
% %% As a result, $\vertiii{\bar{Y}_i}_{\Psi_2} \leq \frac{K\|\theta\|_2}{1-\phi}$. 
% %% 
% %
% %
% %
% %
% %Note that, by jensen inequality, $E[\exp\{\langle Z_i, \theta \rangle \}] \geq \exp\{E[\langle Z_i, \theta \rangle ]\}$.
% %Let $\bar{Y}_m \in \R^m$, for some $m \leq n_q$, be the vector whose elemens are of the form $\bar{Y}_i$ corresponding to $m$ independent samples $Z_i$. In particular, for any $\alpha \in (0,1)$, let $m \geq (1-\alpha)(1-\phi)n_q = \pi n_q$, where $\pi = (1-\alpha)(1-\phi)$.
% %%, after
% %Applying the Hoeffding-type inequality for sub-Gaussian variables \cite[Proposition 5.10]{vers12}, we have
% %\begin{align}
% % P\left(\sum_{j\neq i} \exp\{\langle Z_i, \theta \rangle \} \I(|\langle Z_i, \theta \rangle| \leq T) \geq (m-1)\beta \right) &\leq e \cdot \exp\{\frac{-4(m-1)^2 \beta^4}{(m-1)}\} \\
% % &= e \cdot \exp\{-4(m-1) \beta^4\}
% %\end{align}
% %Let
% %\begin{align}
% %\sum_{i=1}^{n_q} \exp\{\langle Z_i, \theta \rangle \} & = \sum_{i=1}^{n_q} \exp\{\langle Z_i, \theta \rangle \} \I(|\langle Z_i, \theta \rangle| \leq T) + \sum_{i=1}^{n_q} \exp\{\langle Z_i, \theta \rangle \} \I(|\langle Z_i, \theta \rangle| \geq T) \\
% %& \leq \pi n_q e^T + (1-\pi) n_q \ell
% %\end{align}
% %% therefore
% %% \begin{align}
% %%  P & \left(\sum_{i=1}^{n_q} \exp\{\langle Z_i, \theta \rangle \} \geq n e^T \right) \\
% %%  & =  P \left \{ \sum_{i=1}^{n_q} \exp\{\langle Z_i, \theta \rangle \} \I(|\langle Z_i, \theta \rangle| \leq T) \geq \frac{1}{2} n e^T \right\} \\
% %% %& \quad \quad P \left\{\bar{M}_{\theta}(Z) \geq (1-\alpha)(1-\phi)n_q \right\} \\
% %% & \phantom{=} ~+
% %% P \left \{ \sum_{i=1}^{n_q} \exp\{\langle Z_i, \theta \rangle \} \I(|\langle Z_i, \theta \rangle| \leq T) \geq \frac{1}{2} n e^T \right\} \\
% %% %& \quad \quad P \left\{ \bar{M}_{\theta}(Z) < (1-\alpha)(1-\phi)n_q \right\}\\
% %% \end{align}
% %
% %
% %
% %
% %
% %
% %\begin{align}
% % P & \left(\sum_{i=1}^{n_q} \exp\{\langle Z_i, \theta \rangle \} \geq \pi n_q e^T \right) \\
% % & =  P \left \{ \sum_{i=1}^{n_q} \exp\{\langle Z_i, \theta \rangle \} \geq \pi n_q e^T \bigg| \bar{M}_{\theta}(Z) \geq (1-\alpha)(1-\phi)n_q \right\} \\
% %& \quad \quad P \left\{\bar{M}_{\theta}(Z) \geq (1-\alpha)(1-\phi)n_q \right\} \\
% %& \phantom{=} ~+
% %P \left \{ \sum_{i=1}^{n_q} \exp\{\langle Z_i, \theta \rangle \} \geq \pi n_q e^T \bigg| \bar{M}_{\theta}(Z) < (1-\alpha)(1-\phi)n_q \right\} \\
% %& \quad \quad P \left\{ \bar{M}_{\theta}(Z) < (1-\alpha)(1-\phi)n_q \right\}\\
% %\end{align}
% %
% %By application of Chernoff bounds for binomial distributions
% %\beq
% %P \left\{ \bar{M}_{\theta}(Z) < (1-\alpha)(1-\phi)n_q \right\} \leq \exp\left( - \frac{\alpha^2 (1-\phi)}{2}n_q \right)
% %\eeq
% %
% %Noting that we are looking for an upper bound
% %\begin{align}
% % P & \left(\sum_{i=1}^{n_q} \exp\{\langle Z_i, \theta \rangle \} \geq \pi n_q e^T \right) \\
% % & =  P \left \{ \sum_{i=1}^{n_q} \exp\{\langle Z_i, \theta \rangle \} \geq \pi n_q e^T \bigg| \bar{M}_{\theta}(Z) \geq (1-\alpha)(1-\phi)n_q \right\} \\
% %& \phantom{=} ~+
% % P \left\{ \bar{M}_{\theta}(Z) < (1-\alpha)(1-\phi)n_q \right\}\\
% %& =  P \left \{ \sum_{i=1}^{n_q} \exp\{\langle Z_i, \theta \rangle \} \geq \pi n_q e^T \bigg| \bar{M}_{\theta}(Z) \geq (1-\alpha)(1-\phi)n_q \right\} \\
% %& \phantom{=} ~+
% %\exp\left( - \frac{\alpha^2 (1-\phi)}{2}n_q \right)\\
% %\end{align}
% %
% %
% %Note that
% %\begin{align}
% % \sigma_i \geq \bar{\sigma}_i =  \frac{\exp\{ \langle Z_i, \theta \rangle \}\I(|\langle Z_i, \theta \rangle| \leq T)}{\sum_{j=1}^{n_q}  \exp\{ \langle Z_j, \theta \rangle \} \I(|\langle Z_i, \theta \rangle| \leq T)} \geq \frac{e^{-T}}{m e^{T}} = \frac{e^{-2T}}{m},
% %\end{align}
% %where the first inequality is the result of
% %\begin{align}
% %\sum_{i=1}^{n_q} \exp\{\langle Z_i, \theta \rangle \} \I(|\langle Z_i, \theta \rangle| \leq T) \leq m e^{T}.
% %\end{align}
% %
% %
% %For convenience, let $\pi = (1-\alpha)(1-\phi)$. Now, based on the $n_q$ samples $Z_i$, consider the discrete random variable $\bar{M}_{\theta}(Z)= |M_{\theta}(Z)|$, where $|.|$ denotes size of a set. Clearly, $\bar{M}_{\theta}(Z) \in \{0,1,\ldots, n_q \}$ follows a binomial distribution with success probability greater than $(1-\phi)$ and $E[\bar{M}_{\theta}(Z)] \geq (1-\phi)n_q$. Then, we have
% %\begin{align*}
% %P & \left\{{\sigma}_i \geq \frac{e^{-2T}}{\pi n_q} \right\} \\
% %& =  P \left \{  {\sigma}_i \geq \frac{e^{-2T}}{\pi n_q} \bigg| \bar{M}_{\theta}(Z) \geq (1-\alpha)(1-\phi)n_q \right\} \\
% %& \quad \quad P \left\{\bar{M}_{\theta}(Z) \geq (1-\alpha)(1-\phi)n_q \right\} \\
% %& \phantom{=} ~+
% %P \left \{  {\sigma}_i \geq \frac{e^{-2T}}{\pi n_q} \geq \frac{t}{2} \bigg|\bar{M}_{\theta}(Z) < (1-\alpha)(1-\phi)n_q \right\} \\
% %& \quad \quad P \left\{ \bar{M}_{\theta}(Z) < (1-\alpha)(1-\phi)n_q \right\}\\
% %\end{align*}
% %
% %By application of Chernoff bounds for binomial distributions
% %\beq
% %P \left\{ \bar{M}_{\theta}(Z) < (1-\alpha)(1-\phi)n_q \right\} \leq \exp\left( - \frac{\alpha^2 (1-\phi)}{2}n_q \right)
% %\eeq
% %
% %Noting that we are looking for an upper bound
% %\begin{align*}
% %P & \left\{{\sigma}_i \geq \frac{e^{-2T}}{\pi n_q} \right\} \\
% %& =  P \left \{  {\sigma}_i \geq \frac{e^{-2T}}{\pi n_q} \bigg| \bar{M}_{\theta}(Z) \geq (1-\alpha)(1-\phi)n_q \right\} \\
% %& \phantom{=} ~+ P \left\{ \bar{M}_{\theta}(Z) < (1-\alpha)(1-\phi)n_q \right\}\\
% %& = P \left \{  {\sigma}_i \geq \frac{e^{-2T}}{\pi n_q} \bigg| \bar{M}_{\theta}(Z) \geq (1-\alpha)(1-\phi)n_q \right\} \\
% %& \phantom{=} ~+ \exp\left( - \frac{\alpha^2 (1-\phi)}{2}n_q \right)
% %\end{align*}
% %
% %
% %\begin{align}
% % \sum_{i=1}^{n_q} \exp\{\langle Z_i, \theta \rangle \} \geq \sum_{i=1}^{n_q} \exp\{\langle Z_i, \theta \rangle \} \I(|\langle Z_i, \theta \rangle| \leq T) \geq m e^{-T}.
% %\end{align}
% %As a result, 
% %\begin{align}
% % \bar{\sigma}_i =  \frac{\exp\{ \langle Z_i, \theta \rangle \}\I(|\langle Z_i, \theta \rangle| \leq T)}{\sum_{j=1}^{n_q}  \exp\{ \langle Z_j, \theta \rangle \}} \leq \frac{e^{T}}{m e^{-T}} = \frac{1}{m e^{-2T}}
% %\end{align}
% %
% %
% %For convenience, let $\pi = (1-\alpha)(1-\phi)$. Now, based on the $n_q$ samples $Z_i$, consider the discrete random variable $\bar{M}_{\theta}(Z)= |M_{\theta}(Z)|$, where $|.|$ denotes size of a set. Clearly, $\bar{M}_{\theta}(Z) \in \{0,1,\ldots, n_q \}$ follows a binomial distribution with success probability greater than $(1-\phi)$ and $E[\bar{M}_{\theta}(Z)] \geq (1-\phi)n_q$. Then, we have
% %\begin{align*}
% %P & \left\{ \bar{\sigma}_i \leq \frac{1}{\pi n_q e^{-2T}} \right\} \\
% %& =  P \left \{  \bar{\sigma}_i \leq \frac{1}{\pi n_q e^{-2T}} \bigg| \bar{M}_{\theta}(Z) \geq (1-\alpha)(1-\phi)n_q \right\} \\
% %& \quad \quad P \left\{\bar{M}_{\theta}(Z) \geq (1-\alpha)(1-\phi)n_q \right\} \\
% %& \phantom{=} ~+
% %P \left \{  \bar{\sigma}_i \leq \frac{1}{\pi n_q e^{-2T}} \geq \frac{t}{2} \bigg|\bar{M}_{\theta}(Z) < (1-\alpha)(1-\phi)n_q \right\} \\
% %& \quad \quad P \left\{ \bar{M}_{\theta}(Z) < (1-\alpha)(1-\phi)n_q \right\}\\
% %\end{align*}
% %
% %
% %
% %% Similarly, let $\bar{\alpha}_i = \exp\{\langle Z_i, \theta \rangle \} \I(|\langle Z_i, \theta \rangle| \leq T)$.
% %% \begin{align}
% %%  P(\bar{\alpha}_i = e^y) = \frac{P\left(e^{\langle Z_i, \theta \rangle} = e^y\right) \I(|\langle Z_i, \theta \rangle| \leq T)}{P\left(|\langle Z_i, \theta \rangle| \leq T\right)} \leq \frac{1}{1-\phi} P\left(e^{\langle Z_i, \theta \rangle} = y\right).
% %% \end{align}
% %
% %Note that, $\bar{\alpha}_i \in \{0, [e^{-T}, e^T]\}$. Define $\beta = e^{-T}$. Therefore, $\bar{\alpha}_i$ is a bounded sub-Gaussian random variable with $\vertiii{\bar{\alpha}_i}_{\Psi_2} \leq \frac{1}{\beta}$.
% %Define $\delta_j = e^\alpha_j - E[e^\alpha_j]$, where $\vertiii{\delta_i}_{\Psi_2} \leq \frac{2}{\beta}$.
% %Applying the Hoeffding-type inequality for centered sub-Gaussian variables \cite[Proposition 5.10]{vers12}, we have
% %\begin{align}
% % P\left(\sum_{j\neq i} \delta_j \geq (m-1)\beta \right) &\leq e \cdot \exp\{\frac{-4(n-1)^2 \beta^4}{(n-1)}\} \\
% % &= e \cdot \exp\{-4(n-1) \beta^4\}
% %\end{align}
% %
% %
% %
% %
% %Let $\bar{\sigma} \in \R^{n_q}$ be the vector whose elemens are $\bar{\sigma_i} = \sigma_i \I(|\langle Z_i, \theta \rangle| \leq T) $, implying that some elemens can be zero. Note that, 
% %\begin{align}
% % \|\sigma\|_2^2 = \sum_{i=1}^{n_q} \sigma_i^2 \geq \sum_{i=1}^{n_q} \bar{\sigma_i}^2 = \|\bar{\sigma}\|_2^2. 
% %\end{align}
% %
% %
% %\newpage
% %
% %Define $\alpha_i = \langle Z_i, \theta \rangle - E[\langle Z_i, \theta \rangle]$, which is a centered sub-Gaussian variable with norm $\vertiii{\alpha_i}_{\Psi_2} \leq 2 \vertiii{\langle Z_i, \theta \rangle}_{\Psi_2} \leq 2 \underbrace{K \|\theta\|_2}_{k}$. Applying the concentration bound for sub-Gaussian random variable, we have
% %\begin{align}
% % P\left(\left| \alpha_i \right| \geq \tau \right) \leq e \cdot \exp\left( - \frac{\tau^2}{4k^2} \right).
% %\label{eq:bndAlpha}
% %\end{align}
% %Thus, with probability at least $1-e \cdot \exp\left( - \frac{\tau^2}{4k^2} \right)$, we have $\alpha_i \in [-\tau, \tau]$.
% %
% %Next, we show that with high probability $\sigma_i$ is a bounded sub-Gaussian.
% %
% %\begin{align}
% % P \left(\sigma_i > \frac{\beta^2}{n} \right) &= P\left( e^{\alpha_i} > \beta ~~\& ~~ \sum_{j\neq i} e^\alpha_j< (n-1)\beta \right) \\
% % &= P\left( e^{\alpha_i} > \beta \right) + P\left(\sum_{j\neq i} e^\alpha_j < (n-1)\beta \right) - 1
% %\end{align}
% %
% %
% %
% %{\bf 1. Bound on $P\left( e^{\alpha_i} > \beta \right)$:}
% %
% %First note that based on Lemma \ref{lem:innprodsubgvec}, $\langle Z_i, \theta \rangle$ is a sub-Gaussian variable with $\vertiii{\langle Z_i, \theta \rangle}_{\Psi_2} \leq \underbrace{K \|\theta\|_2}_{k}$. %Given that $\| \theta \|_2 < c$,
% %Note that $E[|\langle Z_i, \theta \rangle|] \leq k$ that is obtained from the definition of sub-Gaussian random variable (Definition \ref{def:subgvar}).
% %Applying the concentration bound for sub-Gaussian random variable, we have
% %\begin{align}
% % P\left(\left| \langle Z_i, \theta \rangle \right| - E[\left| \langle Z_i, \theta \rangle \right|] \geq \tau \right) 
% %\leq e \cdot \exp\left( - \frac{\tau^2}{4k^2} \right)
% %\label{eq:bndAlpha}
% %\end{align}
% %set $\tau=2k$, we have
% %\begin{align}
% % P\left(\left| \langle Z_i, \theta \rangle \right| \geq \tau \right) 
% %\leq e \cdot \exp\left( - \frac{\tau^2}{k^2} \right).
% %\label{eq:bndAlpha}
% %\end{align}
% %
% %
% %
% %{\bf Bound on $P\left(\sum_{j\neq i}\alpha_j < (n-1)\beta \right)$:}
% %
% %Note that
% %\begin{align}
% % & P\left( -\tau \leq \alpha_j \leq \tau \right) \geq 1-e \cdot \exp\left( - \frac{\tau^2}{4k^2} \right) \\
% % \Rightarrow & P\left( e^{-\tau} \leq \alpha_j \leq e^{\tau} \right) \geq 1-e \cdot \exp\left( - \frac{\tau^2}{4k^2} \right) 
% %\end{align}
% %Define $\beta = e^{-\tau}$. Therefore, $e^{\alpha_j}$ is a bounded sub-Gaussian with $\vertiii{e^{\alpha_j}}_{\Psi_2} \leq \frac{1}{\beta}$.
% %Define $\delta_j = e^\alpha_j - E[e^\alpha_j]$, where $\vertiii{\delta_i}_{\Psi_2} \leq \frac{2}{\beta}$.
% %Applying the Hoeffding-type inequality for centered sub-Gaussian variables \cite[Proposition 5.10]{vers12}, we have
% %\begin{align}
% % P\left(\sum_{j\neq i} \delta_j \geq (n-1)\beta \Big\| |\alpha_j\right) &\leq e \cdot \exp\{\frac{-4(n-1)^2 \beta^4}{(n-1)}\} \\
% % &= e \cdot \exp\{-4(n-1) \beta^4\}
% %\end{align}
% %
% 
% 
% 
% 
% 
% 
% % \newpage
% % 
% % \begin{lemma}
% % Let $\sigma_i = \hat{r}(X_i^q|\theta) = \frac{\exp\{ \langle Z_i, \theta \rangle \}}{\sum_{j=1}^{n_q}  \exp\{ \langle Z_j, \theta \rangle \}}$. 
% % Assume $\|\theta\|_2 < c$. Then, for $\pi n_q > \eta_3 \tau^2$ with probability at least, $1-e \cdot \exp\left(-\tau^2 \eta_2 \right)$, we have % - \exp\left(-n \eta_1\right)$, we have
% % \begin{align}
% % \frac{1}{\pi n_q} \leq \sigma_i \leq \frac{e^{2\tau}}{\pi n_q},
% % \end{align}
% % where $\alpha\in(0,1)$, and $\pi = (1-\alpha)(1-\phi)$, $\phi = P\left(|\langle Z_i, \theta \rangle| \geq \tau\right) \leq e \cdot \exp\left( - \eta_2 \tau^2 \right)$, and $\eta_2=\frac{1}{4\|\theta\|_2K}$ is a positive constant and $\eta_3$ is a positive constant depends on $\eta_2$ and $\alpha$.
% % \label{lem:bndsig}
% % \end{lemma}
% % % $\eta_1$ is a constant depends on $\pi$, and 
% % 
% % \proof
% % First note that based on Lemma \ref{lem:innprodsubgvec}, $\langle Z_i, \theta \rangle$ is a sub-Gaussian variable with $\vertiii{\langle Z_i, \theta \rangle}_{\Psi_2} \leq \underbrace{K \|\theta\|_2}_{k}$. %Given that $\| \theta \|_2 < c$,
% % %Note that $E[|\langle Z_i, \theta \rangle|] \leq k$ that is obtained from the definition of sub-Gaussian random variable (Definition \ref{def:subgvar}).
% % Applying the concentration bound for sub-Gaussian random variable, we have
% % \begin{align}
% %  P\left(\left| \langle Z_i, \theta \rangle \right| - E[\left| \langle Z_i, \theta \rangle \right|] \geq \tau \right) 
% % \leq e \cdot \exp\left( - \frac{\tau^2}{4k^2} \right).
% % \label{eq:bndAlpha}
% % \end{align}
% % %set $\tau=2k$, we have
% % %\begin{align}
% % %&  P\left(\left| \langle Z_i, \theta \rangle \right| \geq \tau \right) \leq e \cdot \exp\left( - \frac{\tau^2}{k^2} \right) \\
% % %\Rightarrow & P\left(\exp\{ \left| \langle Z_i, \theta \rangle \right| \} \geq e^\tau \right) \leq e \cdot \exp\left( - \frac{\tau^2}{k^2} \right).
% % %\label{eq:bndAlpha}
% % %\end{align}
% % 
% % Let $Y_i(\theta) = \langle Z_i, \theta \rangle - E[\langle Z_i, \theta \rangle]$.
% % Define the event $M_{\theta}(Z) = \{Z_i: |Y_i(\theta)| \leq \tau \}$. 
% % %%Define $Y_i = \langle Z_i, \theta \rangle$, which is a sub-Gaussian random variable with norm $\vertiii{Y_i}_{\Psi_2} \leq K \|\theta\|_2$. 
% % Now, for any fixed $\tau$, let $\bar{Y_i} = Y_i(\theta) \I(|Y_i(\theta)| \leq \tau)$.
% % Let $\bar{Y}_m \in \R^m$, for some $m \leq n_q$, be the vector whose elemens are of the form $\bar{Y}_i$ corresponding to $m$ independent samples $Z_i$.
% % 
% % Using the definition of the $\sigma$, for any $m$, 
% % \begin{align}
% %  \sigma_i =  \frac{\exp\{ \langle Z_i, \theta \rangle \}}{\sum_{j=1}^{n_q}  \exp\{ \langle Z_j, \theta \rangle \}} = \frac{\exp\{ \langle Z_i, \theta \rangle - E[\langle Z_i, \theta \rangle] \}}{\sum_{j=1}^{n_q}  \exp\{ \langle Z_j, \theta \rangle -E[\langle Z_i, \theta \rangle] \}} \leq \frac{Y_i(\theta)}{m e^{-\tau}},
% %  \label{eq:uppbndsigGivm}
% % \end{align}
% % since
% % \begin{align}
% % \sum_{i=1}^{n_q} \exp\{\langle Z_i, \theta \rangle - E[\langle Z_i, \theta \rangle] \} = \sum_{i=1}^{n_q}  \exp\{Y_i(\theta)\} \geq \sum_{i=1}^{n_q}  \exp\{Y_i(\theta)\} \I(|Y_i(\theta)| \leq \tau) \geq m e^{-\tau}.
% % \end{align}
% % 
% % For convenience, let $\pi = (1-\alpha)(1-\phi)$ where $\phi = P\left(Y_i(\theta)| \geq \tau\right) \leq e \cdot \exp\left( - \tau^2/(4k^2) \right)$. As a result, using \eqref{eq:bndAlpha} and \eqref{eq:uppbndsigGivm}, for any $m> \pi n_q$, we get the upper bound on $\sigma_i$, 
% % \begin{align}
% % P\left( \sigma_i \leq \frac{e^{\tau}}{\pi n_q e^{-\tau}}\right) = P\left( \exp\{Y_i(\theta)\} \leq e^\tau \right) \geq 1-e \cdot \exp\left( - \frac{\tau^2}{4k^2} \right).
% % \end{align}
% % 
% % Now, based on the $n_q$ samples $Z_i$, consider the discrete random variable $\bar{M}_{\theta}(Z)= |M_{\theta}(Z)|$, where $|.|$ denotes size of a set. Clearly, $\bar{M}_{\theta}(Z) \in \{0,1,\ldots, n_q \}$ follows a binomial distribution with success probability greater than $(1-\phi)$ and $E[\bar{M}_{\theta}(Z)] \geq (1-\phi)n_q$. Then, we have
% % \begin{align}
% %  P & \left(\sigma_i \geq \frac{e^{\tau}}{\pi n_q e^{-\tau}} \right) \\
% %  & =  P \left \{ \sigma_i \geq \frac{e^{\tau}}{\pi n_q e^{-\tau}} \bigg| \bar{M}_{\theta}(Z) \geq (1-\alpha)(1-\phi)n_q \right\} \\
% % & \quad \quad P \left\{\bar{M}_{\theta}(Z) \geq (1-\alpha)(1-\phi)n_q \right\} \\
% % & \phantom{=} ~+
% % P \left \{ \sigma_i \geq \frac{e^{\tau}}{\pi n_q e^{-\tau}} \bigg| \bar{M}_{\theta}(Z) < (1-\alpha)(1-\phi)n_q \right\} \\
% % & \quad \quad P \left\{ \bar{M}_{\theta}(Z) < (1-\alpha)(1-\phi)n_q \right\}\\
% % \end{align}
% % 
% % By application of Chernoff bounds for binomial distributions
% % \beq
% % P \left\{ \bar{M}_{\theta}(Z) < (1-\alpha)(1-\phi)n_q \right\} \leq \exp\left( - \frac{\alpha^2 (1-\phi)}{2}n_q \right)
% % \eeq
% % 
% % Noting that we are looking for an upper bound
% % \begin{align}
% %  P & \left(\sigma_i \geq \frac{e^{\tau}}{\pi n_q e^{-\tau}} \right) \\
% %  & =  P \left \{ \sigma_i \geq \frac{e^{\tau}}{\pi n_q e^{-\tau}} \bigg| \bar{M}_{\theta}(Z) \geq (1-\alpha)(1-\phi)n_q \right\} \\
% % & \phantom{=} ~+
% %  P \left\{ \bar{M}_{\theta}(Z) < (1-\alpha)(1-\phi)n_q \right\}\\
% %  & \leq e \cdot \exp\left( - \frac{\tau^2}{4k^2} \right) + \exp\left( - \frac{\alpha^2 (1-\phi)}{2}n_q \right).
% % \end{align}
% % 
% % Similarly, we can show that,  using \eqref{eq:bndAlpha} and \eqref{eq:uppbndsigGivm}, for any $m> \pi n_q$, we have
% % \begin{align}
% % P\left( \sigma_i \leq \frac{e^{-\tau}}{\pi n_q e^{-\tau}}\right) = P\left( \exp\{Y_i(\theta)\} \leq e^{-\tau} \right) \leq e \cdot \exp\left( - \frac{\tau^2}{4k^2} \right).
% % \end{align}
% % and considering all value of $m$, we have
% % \begin{align}
% %  P & \left(\sigma_i \leq \frac{1}{\pi n_q} \right) \\
% %  & =  P \left \{ \sigma_i \leq \frac{1}{\pi n_q} \bigg| \bar{M}_{\theta}(Z) \geq (1-\alpha)(1-\phi)n_q \right\} \\
% % & \phantom{=} ~+
% %  P \left\{ \bar{M}_{\theta}(Z) < (1-\alpha)(1-\phi)n_q \right\}\\
% %  & \leq e \cdot \exp\left( - \frac{\tau^2}{4k^2} \right) + \exp\left( - \frac{\alpha^2 (1-\phi)}{2}n_q \right) \\
% %  & \leq e \cdot \exp\left(-\tau^2 \eta_2 \right) + \exp\left( - \eta_1 n_q \right) \\
% %  & \leq e \cdot \exp\left(-\tau^2 \eta_2 \right).
% % \end{align}
% % for $n_q>\frac{\eta_2}{\eta_1}\tau^2$ or equivalently $\pi n_q > \frac{2 (\alpha-1) \eta_2}{(\alpha^2}\tau^2$ where $\eta_1 = \frac{\alpha^2 (1-\phi)}{2}$, $\eta_2=\frac{1}{4\|\theta\|_2K}$. 
% % Setting $\eta_3 = \frac{2 (1-\alpha) \eta_2}{\alpha^2}$ completes the proof.
% % \qed
% % 
% % \newpage
% % 
% % 
% % %Note that $E[\sigma_i] = \frac{\sum_{i=1}^{n_q} \sigma_i}{n_q} = \frac{1}{n_q}$. 
% % \begin{lemma}
% % Let $\sigma_i = \hat{r}(X_i^q|\theta) = \frac{\exp\{ \langle Z_i, \theta \rangle \}}{\sum_{j=1}^{n_q}  \exp\{ \langle Z_j, \theta \rangle \}}$. 
% % Assume $\|\theta\|_2 < c$. Then, for $n>\frac{\eta_2}{\eta_1}\tau^2$ with probability at least $1- e^{2} \cdot \exp\left( -4c_2 - \tau^2 \eta_2 \right)$, we have
% % \begin{align}
% % \|w\|_2 < \frac{ce^{4\tau}}{ \pi\sqrt{n_q}},
% % \end{align} 
% % where $\pi = (1-\alpha)(1-\phi)$, and $\eta_2=\frac{1}{4\|\theta\|_2K}$, and $\alpha \in (0,1)$ is a positive constant.
% % \end{lemma}
% % 
% % \proof
% % Let $\beta= e^{-2\tau}\sqrt{\pi}$. Given that $\sigma_i \in \left( \frac{1}{\pi n_q}, \frac{1}{n_q\beta^2} \right)$ is bounded with $E[\sigma_i] = \frac{1}{n_q}$. Therefore, $\sigma_i^2 \in \left(\frac{1}{\pi^2 n_q^2}, \frac{1}{n_q^2\beta^4} \right)$ is a sub-Gaussian variable with $\vertiii{\sigma_i^2}_{\Psi_2} < \frac{1}{n_q^2\beta^4}$ and $E[\sigma_i^2] \leq \frac{1}{n_q^2\beta^4}$. Applying Lemma \ref{lem:sumsubgvar}, we have $\vertiii{\sum_{i=1}^{n_q} \sigma_i^2 - E[\sigma_i^2]}_{\Psi_2} < n_q\frac{1}{n_q^2\beta^4} = \frac{1}{n_q\beta^4}$. 
% % %Using the triangle inequality, $\vertiii{\sum_{i=1}^{n_q} \sigma_i^2 - E[\sigma_i^2]}_{\Psi_2} < n_q\frac{1}{2n_q^2\beta^4} = \frac{1}{2n_q\beta^4}$
% % 
% % %{\color{red} check if it is true! In particular if $X_1$ and $X_2$ are dependent sub-exponential random variable with $\vertiii{X_1}_{\Psi_1}=\vertiii{X_2}_{\Psi_1} = K$, then $X_1+X_2$ is a sub-exponential random variable with $\vertiii{X_1+X_2}_{\Psi_1} = 2K$. Check Lemma \ref{lem:subExp} as an initial proof of this argument}.
% % 
% % With the concentration bound on sub-Gaussian random variables, we have
% % \begin{align}
% % p \left(|\sum_{i=1}^{n_q} \sigma_i^2 - E[\sigma_i^2]| > \epsilon ~~\Big |~~ \forall i \sigma_i \in \left( \frac{1}{\pi n_q}, \frac{1}{n_q\beta^2} \right) \right) 
% % &\leq 
% % e \cdot \exp \left\{- \frac{c_2\epsilon^2}{\vertiii{\sum_{i=1}^{n_q} \sigma_i^2 - E[\sigma_i^2]}_{\Psi_2}^2} \right \} \\ 
% % &= e \cdot \exp \left\{- 4c_2 \epsilon^2 n_q^2 \beta^8 \right \}
% % \end{align}
% % Setting $\epsilon = \frac{1}{\beta^2 n_q}$, we have
% % 
% % \beq
% % p \left (|\sum_{i=1}^{n_q} \sigma_i^2 - E[\sigma_i^2]| > \frac{1}{\beta^2 n_q} ~~\Big |~~ \forall i \sigma_i \in \left( \frac{1}{\pi n_q}, \frac{1}{n_q\beta^2} \right) \right) \leq e \cdot \exp \left\{ -4c_2 \right \}
% % \label{eq:condBndW}
% % \eeq
% % 
% % 
% % % Note that 
% % % \begin{align}
% % %  P\left( \forall i \sigma_i \in \left( \frac{1}{\pi n_q}, \frac{1}{n_q\beta^2} \right) \right) & = 1 - P\left(\exists \sigma_i  \not\in \left( \frac{1}{\pi n_q}, \frac{1}{n_q\beta^2} \right) \right) \\
% % %  & \leq 1 - 
% % % \end{align}
% % 
% % Putting the result of Lemma \ref{lem:bndsig} and \eqref{eq:condBndW} together, we have
% % \begin{align}
% % p & \left (|\sum_{i=1}^{n_q} \sigma_i^2-E[\sigma_i^2]| > \frac{1}{\beta^4 n_q} \right) \\
% % & = p \left (|\sum_{i=1}^{n_q} \sigma_i^2 - E[\sigma_i^2]| > \frac{1}{\beta^2 n_q} ~~\Big |~~ \forall i \sigma_i \in \left( \frac{1}{\pi n_q}, \frac{1}{n_q\beta^2} \right) \right) \\
% % & \quad \quad P\left( \forall i \sigma_i \in \left( \frac{1}{\pi n_q}, \frac{1}{n_q\beta^2} \right) \right) \\
% % & \phantom{=} ~+
% % p \left (|\sum_{i=1}^{n_q} \sigma_i^2 - E[\sigma_i^2]| > \frac{1}{\beta^2 n_q} ~~\Big |~~ \exists \sigma_i  \not\in \left( \frac{1}{\pi n_q}, \frac{1}{n_q\beta^2} \right) \right) \\
% % & \quad \quad P\left( \exists \sigma_i  \not\in \left( \frac{1}{\pi n_q}, \frac{1}{n_q\beta^2} \right) \right) \\
% % \label{eq:BndWE}
% % \end{align}
% % 
% % 
% % Note that we are looking for an upper bound,
% % \begin{align}
% % p & \left (|\sum_{i=1}^{n_q} \sigma_i^2-E[\sigma_i^2]| > \frac{1}{\beta^4 n_q} \right) \\
% % & = p \left (|\sum_{i=1}^{n_q} \sigma_i^2 - E[\sigma_i^2]| > \frac{1}{\beta^2 n_q} ~~\Big |~~ \forall i \sigma_i \in \left( \frac{1}{\pi n_q}, \frac{1}{n_q\beta^2} \right) \right) \\
% % & \phantom{=} ~+
% %  P\left( \exists \sigma_i  \not\in \left( \frac{1}{\pi n_q}, \frac{1}{n_q\beta^2} \right) \right) \\
% %  & \leq e \cdot \exp \left\{ -4c_2 \right \}  P\left( \exists \sigma_i  \not\in \left( \frac{1}{\pi n_q}, \frac{1}{n_q\beta^2} \right) \right) 
% % \label{eq:BndWE}
% % \end{align}
% % 
% % {\color{red} rest of lemma is wrong, since they require on a bound on the last probability.}
% % 
% % One option:
% % Define the bernouli variable $\xi_i = \I (\sigma_i \in \left( \frac{1}{\pi n_q}, \frac{1}{n_q\beta^2} \right))$. Define the event $\xi(\sigma) = \{\sigma_i: \I (\sigma_i \in \left( \frac{1}{\pi n_q}, \frac{1}{n_q\beta^2} \right)) \}$. 
% % Clearly, the discrete variable $|\xi(\sigma)| \in \{0, 1, \cdots n_q\}$ follows a binomial distribution with success probability greater than $1-\exp\{\tau^2 \eta_2 - n \eta_1\}$ and $E[|\xi(\sigma)|] \geq (1-\phi_1) n_q$, where $\phi_1 = \exp\{\tau^2 \eta_2 - n \eta_1\}$. 
% % 
% % By application of Chernoff bounds for binomial distributions
% % \begin{align}
% % P\left(|\xi(\sigma)| < (1-\alpha)(1-\phi_1)n_q \right) \leq \exp\left( -\frac{\alpha^2 (1-\phi)}{2} n_q \right)
% % \end{align}
% % 
% % {\bf But, note that $\sigma_i$ are dependent!}
% % 
% % % Or, we can use the union bound, but the result is not intersting. Putting the result of Lemma \ref{lem:bndsig} and \eqref{eq:condBndW} together, we have
% % % \beq
% % % p \left (|\sum_{i=1}^{n_q} \sigma_i^2-E[\sigma_i^2]| > \frac{1}{\beta^4 n_q} \right) \leq e^{2} \cdot \exp\left( -4c_2 - \tau^2 \eta_2 - n \eta_1 + \log n \right)
% % % \label{eq:BndWE}
% % % \eeq
% % 
% % % Bound on $E[\sum_{i=1}^{n_q} \sigma_i^2]$:
% % % \beq
% % % E[\sum_{i=1}^{n_q} \sigma_i^2] = \sum_{i=1}^{n_q} E[\sigma_i^2] \leq \frac{1}{2n_q\beta^4}
% % % \label{eq:BndEwSq}
% % % \eeq
% % % where the last inequality obtain by using the fact that $\sigma_i$ is a sub-Gaussian with $\vertiii{\sigma_i}_{\Psi_2} < \frac{1}{2n_q\beta^2}$, therefore $E[\sigma_i^2] < 2 \frac{1}{4n_q^2\beta^4} = \frac{1}{2n_q^2\beta^4}$. 
% % % This is from the definition of sub-Gaussian variable for $p =2$: $(E[|X|^p])^{1/p} < \vertiii{X}_{\Psi_2} \sqrt{p}$.
% % 
% % From\eqref{eq:BndWE} and $E[\sigma_i^2] \leq \frac{1}{2n_q^2\beta^4}$, we have
% % \begin{align}
% % p \left (\sum_{i=1}^{n_q} \sigma_i^2 \leq E[\sigma_i^2]+\frac{1}{\beta^4 n_q} \right) \geq 1- e^{2} \cdot \exp\left( -4c_2 - \frac{c_1 \tau^2}{K^2} \right) \\
% % p \left (\sum_{i=1}^{n_q} \sigma_i^2 \leq \frac{3}{2\beta^4 n_q} \right) \geq 1- e^{2} \cdot \exp\left( -4c_2 - \tau^2 \eta_2 \right)
% % \end{align}
% % 
% % Therefore, $\|w\|_2 < \frac{\sqrt{3/2}}{\beta^2 \sqrt{n_q}}$ with probability at least $1- e^{2} \cdot \exp\left( -4c_2 - \tau^2 \eta_2 \right)$.
% % \qed
% 
% % \begin{align}
% % \nabla \cL(\theta^{*}) &= \frac{-1}{n_p} \sum_{i=1}^{n_p} T(X_{i}^p) + \sum_{i=1}^{n_q} T(X_{i}^q) \hat{r}(X|\theta) \nonumber \\
% %  &= \frac{-1}{\sqrt{n_p}} Z_p^Tw_p + Z_q^Tw_q \nonumber \\
% % \end{align}
% % where
% % $Z_p=\{T(X_i^p)\}$, $Z_q=\{T(X_i^q)\}$, $w_q=\{ \hat{r}(X_i^q|\theta)\}$, $w_p=\{\frac{1}{\sqrt{n_p}}, \frac{1}{\sqrt{n_p}}, \cdots , \frac{1}{\sqrt{n_p}}\}$and
% % \begin{align}
% %  \hat{r}(X_i^q|\theta) = \frac{\exp\{ \langle T(X_i^q), \theta_r \rangle \}}{\sum_{i=1}^{n_q}  \exp\{ \langle T(X_i^q), \theta_r \rangle \}}.
% % \end{align}
% % 
% % Then, using the definition of dual norm we have
% % \begin{align}
% % R^*\left(\nabla \cL(\theta^{*}) \right) &= \sup_{R(u)\leq 1} \langle \frac{-1}{\sqrt{n_p}} Z_p^Tw_p + Z_q^Tw_q, u \rangle.
% % \end{align}
% % 
% % % elements of  $w_q$ are bounded between, it has the sub-Gaussian norm less than $\frac{1}{\sqrt{n_q}}$ with probability at least .... 
% % For a given $u$, consider sub-exponential process $\langle Z_q^Tw_q, u \rangle$, with sub-exponential norm as,
% % \begin{align}
% % \vertiii{\langle Z_q^Tw_q, u \rangle}_{\Psi_1} = \vertiii{\langle w_q, Z_q u \rangle}_{\Psi_1} \leq \frac{1}{\sqrt{n_q}} K \|u\|_2,
% % \end{align}
% % where $\vertiii{Z_q^{(i)}}_{\Psi_2} < K$, and since elements of  $w_q$ are bounded, it has the sub-Gaussian norm less than $\frac{1}{\sqrt{n_q}}$ with probability at least .... 
% % 
% % Using the sub-exponential concentration bound, we have
% % \begin{align}
% % P\left(\big|\langle Z_q^Tw_q, u \rangle - E_q[\langle Z_q^Tw_q, u \rangle]\big| \geq \epsilon \right) \leq e \cdot \exp\{ - \min \left( \frac{\epsilon^2n_q}{K^2\|u\|_2^2}, \frac{\epsilon\sqrt{n_q}}{K\|u\|_2} \right) \}.
% % \label{eq:sub-exp-conc}
% % \end{align}
% % 
% % Note that
% % \begin{align}
% % E_q\left[ Z_q^Tw_q \right] =  E_{X_i\sim q}\left[\sum_{i=1}^{n_q} T(X_i^q) r(X_i^q|\theta_r^*)\right]= E_{X\sim q}[T(X) r(X|\theta_r^*)] = E_{X\sim p}[T(X)] 
% % \end{align}
% % where the last equality is based on $r(X|\theta_r^*) q(X|\theta_q^*) = p(X|\theta_p^*)$. Using the linearity of the inner product operator, we have
% % \begin{align}
% % \left \langle E_q[ Z_q^T w_q], ~ u \right \rangle =  E_q\left[\langle Z_q^T w_q, u\rangle \right] = E_{X\sim p}[ \langle T(X)], u \rangle]
% % \label{eq:eqEpEqr}
% % \end{align}
% % Therefore, setting $\epsilon =\frac{w(\Omega_R)}{\sqrt{n_q}}$, and using \eqref{eq:eqEpEqr}, \eqref{eq:sub-exp-conc} can be represented as
% % \begin{align}
% % P\left(\big|\langle Z_q^Tw_q, u \rangle - E_{X\sim p}[ \langle T(X)], u \rangle] \big| \geq \frac{w(\Omega_R)}{\sqrt{n_q}} \right) \leq 2 \exp\{ - \min \left( \frac{w^2(\Omega_R)}{K^2\|u\|_2^2}, \frac{w(\Omega_R)}{K\|u\|_2} \right) \}.
% % \end{align}
% % 
% % As a result, with probability at least $1 - 2 \exp\{ - \min \left( \frac{w^2(\Omega_R)}{K^2\|u\|_2^2}, \frac{w(\Omega_R)}{K\|u\|_2} \right) \}$, we have
% % \begin{align}
% % \frac{w(\Omega_R)}{\sqrt{n_q}}  - \langle \frac{1}{\sqrt{n_p}} Z_p^Tw_p -E_{X\sim p}[ \langle T(X)], u \rangle] \rangle \nonumber \\
% % \leq \langle \frac{1}{\sqrt{n_p}} Z_p^Tw_p - Z_q^Tw_q, u \rangle \leq  \nonumber \\
% % \frac{w(\Omega_R)}{\sqrt{n_q}}  + \langle \frac{1}{\sqrt{n_p}} Z_p^Tw_p - E_{X\sim p}[ \langle T(X)], u \rangle] \rangle
% % \end{align}
% % 
% % As a result,
% % \begin{align}
% % %\sup_{R(u)\leq1} \frac{w(\Omega_R)}{\sqrt{n_q}}  - \langle \frac{1}{\sqrt{n_p}} Z_p^Tw_p -E_{X\sim p}[ \langle T(X)], u \rangle] \rangle \nonumber \\
% % %\leq 
% % \sup_{R(u)\leq1} \langle \frac{1}{\sqrt{n_p}} Z_p^Tw_p - Z_q^Tw_q, u \rangle \leq  
% % \frac{w(\Omega_R)}{\sqrt{n_q}}  +\sup_{R(u)\leq1}   \langle \frac{1}{\sqrt{n_p}} Z_p^Tw_p - E_{X\sim p}[ \langle T(X)], u \rangle] \rangle
% % \end{align}
% % 
% % Now, using Lemma \ref{lem:ExpBndLambdaXp}, with the probability at least .....
% % we have,
% % \begin{align}
% %  \sup_{R(u)\leq1}   \langle \frac{1}{\sqrt{n_p}} Z_p^Tw_p - E_{X\sim p}[ \langle T(X)], u \rangle] \rangle \leq \frac{w(\Omega_R}{\sqrt{n_p}}.
% %  \end{align} 
% %  As a result,
% % \begin{align}
% % \sup_{R(u)\leq1} \langle \frac{1}{\sqrt{n_p}} Z_p^Tw_p - Z_q^Tw_q, u \rangle \leq  
% % \frac{w(\Omega_R)}{\sqrt{n_q}}  + \frac{w(\Omega_R}{\sqrt{n_p}}.
% % \end{align}
% % That completes the proof.
% % 
% % \textbf{Upper bound for $R^*\left(\frac{-1}{n_p} \sum_{i=1}^{n_p} T(X_{i}^p) + E_{X\sim p}[T(X)]\right)$:}
% % % \begin{align}
% % % \nabla \cL(\theta^{*}) &= \frac{-1}{n_p} \sum_{i=1}^{n_p} T(X_{i}^p) + \sum_{i=1}^{n_q} T(X_{i}^q) \hat{r}(X_i^q|\theta) \\
% % %  &= \frac{-1}{\sqrt{n_p}} \langle Z^p, w \rangle + \sum_{i=1}^{n_q} T(X_{i}^q) \hat{r}(X_i^q|\theta) 
% % % \end{align}
% % 
% % \begin{lemma}
% % Consider sub-Gaussian sufficient statistic $T(X_i^p)$ with $\vertiii{T(X_i^p)} _{\Psi_2}< K$ for all $i = 1, \cdots n_p$ where samples $\{X_i^p\}_{i=1}^{n_p}$ are independent. Define $\Omega_R = \{u: R(u) \leq 1\}$. Then, with probability at least {\color{red} find the probability}
% % \begin{align}
% %  R^*\left(\frac{1}{n_p} \sum_{i=1}^{n_p} T(X_{i}^p) - E_{X\sim p}[T(X)] \right) \leq \frac{w(\Omega_R)}{\sqrt{n_p}},
% % \end{align}
% % where $w(\Omega_R)$ is the Gaussian width of set $\Omega_R$.
% % \label{lem:ExpBndLambdaXp}
% % \end{lemma}
% % 
% % \proof
% % Define $Z\in \R^{n_p \times d}$ with each row $Z_i = T(X_{i}^p) - E_{X\sim p}[T(X)]$ is a centered sub-Gaussian vector with $\vertiii{Z_i}_{\Psi_2} < 2K$.
% % Let $w=[\frac{1}{\sqrt{n_p}}, \frac{1}{\sqrt{n_p}}, \cdots , \frac{1}{\sqrt{n_p}}] \in \R^{n_p}$ be a unit length vector.
% % Then using the definition of dual norm, we have
% % \begin{align}
% %  \frac{1}{n_p} R^*\left(\sum_{i=1}^{n_p} T(X_{i}^p) - E_{X\sim p}[T(X)] \right) &= \frac{1}{\sqrt{n_p}} R^*\left(Z^T w\right) \\
% %  &= \frac{1}{\sqrt{n_p}} \sup_{R(u) \leq 1} \left \langle Z^T w, u \right \rangle 
% %  = \frac{1}{\sqrt{n_p}} \sup_{R(u) \leq 1}  \left \langle Z u , w \right \rangle.
% % \end{align}
% % 
% % 
% % Note that $E[Z^Tw] = \frac{1}{\sqrt{n_p}}E[\sum_{i=1}^{n_p} Z_i] = 0$.
% % Next by applying the lemma \ref{lem:subGaussianWidthGaussianWidth}, we have
% % \begin{align}
% % E\left[R^*(\frac{1}{n_p} \sum_{i=1}^{n_p} T(X_{i}^p))\right] = E\left[\frac{1}{\sqrt{n_p}} \sup_{u \in \Omega_R} \left \langle Z u , w \right \rangle \right] \leq  \frac{c_1}{\sqrt{n_p}} w(\Omega_R).
% % \label{eq:}
% % \end{align}
% % 
% % {\color{red} the proof needs to be completed}
% % 
% % 
% % \begin{lemma}
% % Define the sub-Gaussian process $H(u) =  \left \langle Z u , w \right \rangle$ indexed by the set $\Omega_R$, i.e., $u \in \Omega_R$. Consider the zero-mean sub-Gaussian process i.e., $E[H(u)] = 0$. Let $w \in \R^{n}$ be a unit-length vector, and $Z \in \R^{n \times d}$ with independent sub-Gaussian rows $Z_i$ where $\vertiii{Z_i}_{\Psi_2} < K$.
% % Then,
% % \begin{align}
% % E[\sup_{u\in \Omega_R} H(u)] \leq c_1 w(\Omega_R),
% % \label{eq:expsubgwidth}
% % \end{align}
% % and with probability at least $1-\eta_3 \exp\{−\eta_4 \epsilon^2\} $
% % \begin{align}
% % \sup_{u\in \Omega_R} H(u) \leq c_1 w(\Omega_R) + \epsilon,
% % \label{eq:concsubGaussianWidthGaussianWidth}
% % \end{align}
% % where $w(\Omega_R)$ is the Gaussian width of $\Omega_R$.
% % \label{lem:subGaussianWidthGaussianWidth}
% % \end{lemma}
% % \proof
% % First note that $h = Z (u-v)$ is a sub-Gaussian vector where $h_i = \langle Z_i, (u-v) \rangle$ is a sub-Gaussian variable with $\vertiii{h_i}_{\Psi_2} \leq K \|u-v\|_2$ (Lemma \ref{lem:innprodsubgvec}). 
% % % It follows from the definition of sub-Gaussian vectors
% % % \begin{align}
% % %  \vertiii{h_i}_{\Psi_2} =  \|u-v\|_2 \vertiii{\left \langle Z_i, \frac{u-v}{\|u-v\|_2} \right \rangle}_{\Psi_2} \leq \|u-v\|_2 \sup_{s\in S^{p-1}} \langle Z^p_i, s \rangle = \|u-v\|_2 \vertiii{Z_i}_{\Psi_2} \leq K \|u-v\|_2.
% % % \end{align}
% % 
% % Since rows of $Z$ are independent, elements of $h_i$ are independent, therefore the rotation invariance \cite[Lemma 5.9]{vers12}
% % implies that $\vertiii{\langle h, w \rangle}_{\Psi_2}  \leq \|w\|_2 K \|u-v\|_2 = K \|u-v\|_2$ where the last equality achieves because $\|w\|_2 = 1 $. 
% % 
% %  Consider the Gaussian process $G(u) = \langle u, g \rangle$, indexed by the same set, i.e., $u \in \Omega_R$, where $g \sim N (0, \I_{{d} \times {d}})$ is standard Gaussian vector. Now we have,
% % \begin{align}
% %  \vertiii{H(u)-H(v)}_{\psi_2} &= \vertiii{\langle Z (u-v) , w \rangle}_{\psi_2} = \vertiii{\langle h, w \rangle}_{\psi_2} \nonumber \\
% %  & \leq K \| u - v \|_2 = K  E_g[ \| G(u) - G(v) \|_2^2]^{1/2}.
% % \end{align}
% % where $E_g[ \| G(u) - G(v) \|_2^2]^{1/2} = E_g[\| \langle u-v , g \rangle\|_2^2]^{1/2} = \| u - v \|_2$.
% % 
% % Next, by applying the Fernique-Talagrand's comparison theorem in \cite[Theorem 8.2]{vers14}, we have
% % \begin{align}
% % E[\sup_{u\in \Omega_R} H(u)] = E\left[ \sup_{u \in \Omega_R} \left \langle Z u , w \right \rangle \right] = \leq c_2 K E[ \sup_{u\in \Omega_R} G(u)] =  c_1 w(\Omega_R),
% % \end{align}
% % where $c_1 = c_2 K$ with a positive constant $c_2$. This completes proof of \eqref{eq:expsubgwidth}.
% % 
% % {\color{red} complete this part, it is ambigous! Finally, the concentration bound \eqref{eq:concsubGaussianWidthGaussianWidth} can be obtained using the Theorem 5 in \cite{bcfs14}.}
% % %Denote $Y = \sup_{u \in \Omega_R} \left \langle Z u , w \right \rangle $}
% % \qed
% 
% 
% %\newpage
% %
% %\begin{align}
% %\nabla \cL(\theta^{*}) &= \frac{-1}{n_p} \sum_{i=1}^{n_p} T(X_{i}^p) + \sum_{i=1}^{n_q} T(X_{i}^q) \hat{r}(X|\theta) \nonumber \\
% % &= \frac{-1}{\sqrt{n_p}} Z_p^Tw_p + Z_q^Tw_q \nonumber \\
% %\end{align}
% %where
% %$Z_p=\{T(X_i^p)\}$, $Z_q=\{T(X_i^q)\}$, $w_q=\{ \hat{r}(X_i^q|\theta)\}$, $w_p=\{\frac{1}{\sqrt{n_p}}, \frac{1}{\sqrt{n_p}}, \cdots , \frac{1}{\sqrt{n_p}}\}$and
% %\begin{align}
% % \hat{r}(X_i^q|\theta) = \frac{\exp\{ \langle T(X_i^q), \theta_r \rangle \}}{\sum_{i=1}^{n_q}  \exp\{ \langle T(X_i^q), \theta_r \rangle \}}.
% %\end{align}
% %
% %Then, using the definition of dual norm we have
% %\begin{align}
% %R^*\left(\nabla \cL(\theta^{*}) \right) &= \sup_{R(u)\leq 1} \langle \frac{-1}{\sqrt{n_p}} Z_p^Tw_p + Z_q^Tw_q, u \rangle.
% %\end{align}
% %
% %For a given $u$, consider sub-exponential process $\langle Z_q^Tw_q, u \rangle$, with sub-exponential norm as,
% %\begin{align}
% %\vertiii{\langle Z_q^Tw_q, u \rangle}_{\Psi_1} = \vertiii{\langle w_q, Z_q u \rangle}_{\Psi_1} \leq \frac{1}{\sqrt{n_q}} K \|u\|_2,
% %\end{align}
% %where $\vertiii{Z_q^{(i)}}_{\Psi_2} < K$, and since elements of  $w_q$ are bounded between, it has the sub-Gaussian norm less than $\frac{1}{\sqrt{n_q}}$ with probability at least .... 
% %
% %Using the sub-exponential concentration bound, we have
% %\begin{align}
% %P\left(\big|\langle Z_q^Tw_q, u \rangle - E_q[\langle Z_q^Tw_q, u \rangle]\big| \geq \epsilon \right) \leq e \cdot \exp\{ - \min \left( \frac{\epsilon^2n_q}{K^2\|u\|_2^2}, \frac{\epsilon\sqrt{n_q}}{K\|u\|_2} \right) \}.
% %\label{eq:sub-exp-conc}
% %\end{align}
% %
% %Note that
% %\begin{align}
% %& E_{X\sim p}[T(X)] = E_{X\sim q}[T(X) r(X|\theta_r^*)] \\
% %\Rightarrow ~& \frac{1}{\sqrt{n_p}}E_{p}[Z_p^Tw_p]= E_q[Z_q^T w_q] \\
% %\Rightarrow ~&\frac{1}{\sqrt{n_p}}E_{p}[\langle Z_p^Tw_p, u \rangle] = E_q[\langle Z_q^T w_q, u\rangle]
% %\end{align}
% %Therefore, setting $\epsilon =\frac{w(\Omega_R)}{\sqrt{n_q}}$, \eqref{eq:sub-exp-conc} can be represented as
% %\begin{align}
% %P\left(\big|\langle Z_q^Tw_q, u \rangle - \frac{1}{\sqrt{n_p}} E_{p}[Z_p^Tw_p, u \rangle]\big| \geq \frac{w(\Omega_R)}{\sqrt{n_q}} \right) \leq 2 \exp\{ - \min \left( \frac{w^2(\Omega_R)}{K^2\|u\|_2^2}, \frac{w(\Omega_R)}{K\|u\|_2} \right) \}.
% %\end{align}
% %
% %As a result, with probability at least $1 - 2 \exp\{ - \min \left( \frac{\epsilon^2}{K^2\|u\|_2^2}, \frac{\epsilon}{K\|u\|_2} \right)$, we have
% %\begin{align}
% %\epsilon - \langle \frac{1}{\sqrt{n_p}} Z_p^Tw_p - E_{p}[\langle Z_p^Tw_p, u \rangle] \rangle
% %\leq \langle \frac{1}{\sqrt{n_p}} Z_p^Tw_p - Z_q^Tw_q, u \rangle \leq 
% %\epsilon + \langle \frac{1}{\sqrt{n_p}} Z_p^Tw_p - E_{p}[\langle Z_p^Tw_p, u \rangle] \rangle
% %\end{align}
% %
% %
% %\newpage
% %

==> theo-rsc.tex <==
In this Section, we establish the RSC condition for direct change detection estimator \eqref{eq:changeestimateopt}.
%Recall, the RSC condition as follows:
%\begin{align}
%\delta \cL(\delta \theta^{*}, u) & := \cL(\delta \theta^{*} + u) - \cL(\delta \theta^{*}) - \langle \nabla \cL(\delta \theta^{*}), u \rangle \nonumber \\
%& \geq \kappa \|u\|_{2}^{2}
%\end{align}
%for $\forall u \in A_{r}$.
Simplifying the expression and applying mean value theorem twice on the left side of RSC condition \eqref{eq:RSC}, for $\forall \gamma_i \in [0, 1]$, we have
\begin{align}
\delta \cL(\delta \theta^{*}, u) & := \cL(\delta \theta^{*} + u) - \cL(\delta \theta^{*}) - \langle \nabla \cL(\delta \theta^{*}), u \rangle \nonumber \\
& \geq u^T \nabla^2 \cL(\delta \theta^*+\gamma_i u) u.
\end{align}
Thus, the RSC condition depends on the non-linear terms of loss function.
Recall that the nonlinear term, second term, in Loss function \eqref{eq:changeestimateopt} 
%is defined
%\begin{align}
%\cL(\theta_r) &= \frac{-1}{n_p} \sum_{i=1}^{n_p} \langle T(X_i^p), \theta_r \rangle \nonumber \\
%& \quad + \log \frac{1}{n_q} \sum_{i=1}^{n_q} \exp\{ \langle T(X_i^q), \theta_r \rangle \},
%\end{align}
%where the nonlinear term
which is the approximation of the log-partition functions only depends on $n_2$. As a results, only samples of $\mathfrak{X}_2^{n_2}$ affect the RSC conditions. Our analysis is an extension of the results on \cite{bcfs14} using the generic chaining. We show that, the RSC condition is satisfied once samples $n_2$ crosses $w^2(C_r)$ the Gaussian width of restricted error set.

\begin{theo}
Consider sub-Gaussian sufficient statistic $T(X_i^q)$ and $T(X_i^p)$ with independent samples $\{X_i^p\}_{i=1}^{n_p}$, $\{X_j^p\}_{j=1}^{n_p}$.
Let $\vertiii{T(X_i^p)} _{\Psi_2}< K$ and  $\vertiii{T(X_j^q)} _{\Psi_2}< K$ for all $i = 1, \cdots n_p$ and $j=1, \cdots n_q$. Then, for any $A \subseteq S^{d-1}$, and any $\epsilon > 0$, with probability at least $(1-\exp(c - \epsilon^2)-e \cdot \exp\left( -\eta_1 \log n \right))$, we have
\beq
\inf_{u \in A} \delta \cL(\theta^{*}, u) \geq \eta_0 \sqrt{n_q} - \eta_1 w(A) - \eta_2 \epsilon.
\eeq
$\eta_0,\eta_1, \eta_2 > 0$ are absolute constants depending on $K$ and $\Lambda_{\max}(\Sigma_Z)$ the largest eigenvalue of $\Sigma_Z^{-1/2}$. Denote $\Sigma_Z^{-1/2}$ as the covariance structure of sufficient statistics $T(X_i^q)$.
\label{theo:rsc}
\end{theo}

The proof is given in Section \ref{sec:supRSC} of supplement.

